OASum: Large-Scale Open Domain Aspect-based Summarization

Aspect or query-based summarization has recently caught more attention, as it can generate differentiated summaries based on users' interests. However, the current dataset for aspect or query-based summarization either focuses on specific domains, contains relatively small-scale instances, or includes only a few aspect types. Such limitations hinder further explorations in this direction. In this work, we take advantage of crowd-sourcing knowledge on Wikipedia.org and automatically create a high-quality, large-scale open-domain aspect-based summarization dataset named OASum, which contains more than 3.7 million instances with around 1 million different aspects on 2 million Wikipedia pages. We provide benchmark results on OASum and demonstrate its ability for diverse aspect-based summarization generation. To overcome the data scarcity problem on specific domains, we also perform zero-shot, few-shot, and fine-tuning on seven downstream datasets. Specifically, zero/few-shot and fine-tuning results show that the model pre-trained on our corpus demonstrates a strong aspect or query-focused generation ability compared with the backbone model. Our dataset and pre-trained checkpoints are publicly available.

==> tables/oasum_finetune.tex <==
\begin{table*}[t]
    \centering
    \footnotesize
    \resizebox{.90\linewidth}{!}{
            \begin{tabular}{llll}
            \toprule
            \multicolumn{4}{p{1.\linewidth}}{ % $\textsc{l}$
                {
                \textbf{History}:
                Seattle is a seaport city on the West Coast of the United States. It is the seat of King County, Washington.
                The Seattle area was inhabited by Native Americans for at least 4,000 years before the first permanent European settlers.
                Arthur A. Denny and his group of travelers, subsequently known as the Denny Party, arrived from Illinois via Portland, Oregon, on the schooner "Exact" at Alki Point on November 13, 1851.}} \\
            \midrule
            \multicolumn{4}{p{1.\linewidth}}{
                {\textbf{History ; Founding}: It is the seat of King County, Washington. The Seattle area was inhabited by Native Americans for at least 4,000 years before the first permanent European settlers. Arthur A. Denny and his group of travelers, subsequently.}}\\
            \midrule
            \multicolumn{4}{p{1.\linewidth}}{
                {\textbf{History ; Post-war years: aircraft and software}: Growth after World War II was partially due to the local Boeing company, which established Seattle as a center for aircraft manufacturing. The stream of new software, biotechnology, and Internet companies led to an economic revival, which increased the city's population by almost 50,000 between 1990 and 2000. Seattle also has a significant musical history.}}\\
            \midrule
            \multicolumn{4}{p{1.\linewidth}}{
                {\textbf{Geography}: Seattle is situated on an isthmus between Puget Sound (an inlet of the Pacific Ocean) and Lake Washington.}}\\
            \midrule
            \multicolumn{4}{p{1.\linewidth}}{
                {\textbf{Economy}: A major gateway for trade with East Asia, Seattle is the fourth-largest port in North America in terms of container handling . Internet retailer Amazon was founded in Seattle in 1994, and major airline Alaska Airlines is based in SeaTac, Washington, serving Seattle's international airport, Seattle–Tacoma International Airport.}}\\
            \midrule
            \multicolumn{4}{p{1.\linewidth}}{
                {\textbf{Culture}: Between 1918 and 1951, nearly two dozen jazz nightclubs existed along Jackson Street, from the current Chinatown/International District to the Central District. The jazz scene nurtured the early careers of Ray Charles, Quincy Jones.}}\\
            \midrule
            \multicolumn{4}{p{1.\linewidth}}{
                {\textbf{Demographics}: Today, Seattle has high populations of Native, Scandinavian, Asian American and African American people, as well as a thriving LGBT community that ranks sixth in the United States by population.}}\\ 
                
            \bottomrule
            \end{tabular}
    }
\caption{Example of aspect-based summaries constructed from the test set.}
\label{tab:seattle}
\end{table*}


